A Kinetic Theory of Encounter-Based Information Propagation in Multi-Robot Systems

Multi-robot systems cannot assume persistent network connectivity. We study this problem through target tracking, where performance depends on how quickly target information is sensed, transported through the team, and used before it becomes stale. When robots exchange information only through physical encounters, tracking becomes a kinetic information-transport problem: robot motion induces encounters, encounters carry target-state estimates, information age determines staleness, and stale information produces tracking error. This paper develops a kinetic theory of encounter-based information propagation and identifies three limits. The first is an access limit -- information cannot support team-level coordination unless it spreads beyond the robots that sensed it. The second is a staleness limit -- even propagated information loses value as the target moves. The third is a geometry limit -- when target motion outpaces information transport, tracking error approaches a saturation regime where communication improvements alone have diminishing returns. We evaluate the theory through large-scale simulations varying team size, operating area, communication range, and target speed. Results support the proposed access-staleness-geometry decomposition: communication coverage governs the access transition; once information is accessible, tracking error is shaped by target displacement; and this response is locally linear in restricted regimes but nonlinear over broader ranges because of sensing refreshes and bounded geometry. Across controlled sweeps and joint variation, the derived access and staleness coordinates reliably describe tracking performance. Together, these results establish a kinetic-theoretic framework for predicting and designing encounter-based multi-robot systems.

==> tables/design_regime_table.tex <==
\begin{table}[t]
  \centering
  \caption{\textbf{Design interpretation of the kinetic limits.}
  The table translates the access, staleness/value, and geometry/target-dynamics limits into deployment actions. The hypothesis is that different error signatures require different interventions: low $\Lam$ calls for more encounter opportunity, high $\Xnorm$ calls for fresher or more predictive information, and saturation calls for target-dynamics or sensing improvements. The caveat is that these regimes overlap and the coverage transition is an empirical band, not a hard classifier.}
  \label{tab:design_regimes}
  \small
  \begin{tabular}{@{}p{0.17\textwidth}p{0.21\textwidth}p{0.28\textwidth}p{0.25\textwidth}@{}}
    \toprule
    Regime & Signature & Mechanism & Design action \\
    \midrule
    Coverage-limited &
    Low $\Lam$, high normalized error &
    Information does not propagate beyond local sensing and occasional nearby encounters &
    Increase $N$, increase $\rc$, reduce operating area, improve mixing or mobility, or add relay/rendezvous behavior \\
    \addlinespace
    Staleness-limited &
    Adequate $\Lam$ but high $\Xnorm$ and high error &
    Information propagates through the team but arrives after the target has moved too far &
    Reduce AoI, increase sensing frequency, use target-motion prediction/filtering, prioritize fresh estimates, or shorten update paths \\
    \addlinespace
    Geometry/target-dynamics-limited &
    High $\vt$ with saturating error despite communication improvements &
    Target motion and bounded geometry limit the value of old estimates; communication alone has diminishing returns &
    Improve target-dynamics prediction, increase robot speed or sensing radius, use active tracking policies, and reduce reliance on encounters alone \\
    \bottomrule
  \end{tabular}
\end{table}
